LITS: An Optimized Learned Index for Strings (An Extended Version)

Index is an important component in database systems. Learned indexes have been shown to outperform traditional tree-based index structures for fixed-sized integer or floating point keys. However, the application of the learned solution to variable-length string keys is under-researched. Our experiments show that existing learned indexes for strings fail to outperform traditional string indexes, such as HOT and ART. String keys are long and variable sized, and often contain skewed prefixes, which make the last-mile search expensive, and adversely impact the capability of learned models to capture the skewed distribution of string keys. In this paper, we propose a novel learned index for string keys, LITS (Learned Index with Hash-enhanced Prefix Table and Sub-tries). We propose an optimized learned model, combining a global Hash-enhanced Prefix Table (HPT) and a per-node local linear model to better distinguish string keys. Moreover, LITS exploits compact leaf nodes and hybrid structures with a PMSS model for efficient point and range operations. Our experimental results using eleven string data sets show that LITS achieves up to 2.43x and 2.27x improvement over HOT and ART for point operations, and attains comparable scan performance.

==> cover.tex <==
\section*{RESPONSE TO REVIEW COMMENTS}

We would like to thank the meta reviewer and all the reviewers for
their valuable suggestions and comments. We have tried our best to
address the issues raised by the reviews.

In the following, we use (page number, section, paragraph) to indicate
the location of the revised contents, where the page number refers to
the main paper excluding the cover pages on response to review
comments.  In the paper, the revised texts are highlighted with
\revise{blue} color.  For figures and tables with revised contents,
the titles are shown in \revise{blue} color.

Due to space limitations, we have to move or add the following
description in an extended version of the paper~\cite{litstr}: 
%
1) Proof of HPT accuracy theorem; 
%
2) Algorithm listings of search and insert algorithms; 
%
3) Detailed complexity analysis of LITS; 
%
4) Experimental results on three different hardware platforms; 
%
5) Experimental results for zipf distribution; 
%
6) In-depth analysis of space consumption of the learned indexes
compared in our work;
%
7) Experiments on two variants of compact leaf node implementation.  
%
We have included the extended version as the supplemental material in
this submission.  We plan to make it publicly available on arxiv.org.

% proof of HTP accuracy result
% cost analysis
% zipf distribution
% algorithm

\newcommand{\qstart}[1]{\vspace{0.15in}\noindent{\bf #1}}
\newcommand{\qother}[1]{\noindent{\bf #1}}
\newcommand{\answer}[1]{\vspace{0.05in}\noindent{\bf #1}}
\newcommand{\feedbk}[1]{\textcolor{darkgray}{\it Feedback: #1}}

\subsection*{1. Response to Review 2}

% --------
\qstart{R2W1,R2D1,R2D5,R2Revision1.} \emph{Unclear design and
measurement of insert and delete operations for indexes.  Add the
evaluation for all operations, including insert and delete.}
% --------

\answer{Response:}
%
For experimental measurements, Section~\ref{subsec:perf} has already
reported the results for the insert-only workload in
Figure~\ref{fig:CI}(b).  In this revision, we add the description of
the delete-only workload in (p.10, Section~\ref{subsec:setup}, last
paragraph), then report the results of the delete-only workload in the
right-most sub-figure in Figure~\ref{fig:BDEF}.  

For the algorithm description, Section~\ref{subsec:overview} has
already described the search, insert, delete, update, and scan index
operations.  Moreover, in this revision, we add the algorithm listings
of the search and the insert algorithms in Appendix A.2 of the
extended version of the paper~\cite{litstr}.  Furthermore, the source
code of LITS is available at \url{\vldbavailabilityurl}.


% --------
\qstart{R2W2,R2D2,R2Revision2.} \emph{Add the spatio-temporal
complexity for all operations.}
% --------

\answer{Response:}
%
We add Section~\ref{subsec:cost} in p.9 to analyze the time and space
costs of LITS.  For page space constraints, the section summarizes the
results, while the full analysis is described in Appendix A.3 in the
extended version of the paper~\cite{litstr}.


% --------
\qstart{R2W3,R2D3,R2Revision3.} \emph{Unclear application scenarios.}
% --------

\answer{Response:}
%
LITS are optimized for use scenarios where variable-length string keys
are indexed.  However, this point is already quite clear from both the
paper title and the introduction.  Therefore, to our understanding,
the main question in this review comment is whether string keys are
used in real world applications.

To address this comment, we modify (p.1, Section~\ref{Re:R2O3},
Paragraph 1) and cite Facebook workload characterization
studies~\cite{AtikogluXFJP12,CaoDVD20} to show that variable-length
keys are indeed common in the real world.  Moreover, in (p.1,
Section~\ref{Re:R2O3}, last paragraph), we emphasize \emph{string
keys} and \emph{string data sets}. 


% --------
\qstart{R2D4,R2Revision4.} \emph{Add an overview for LITS. The
introduction of LITS structure is fragmented and lacks an overall
introduction; there is a lack of overview of the structure itself,
making it difficult for readers to quickly grasp the macroscopic
structure of LITS.} 
% --------

\answer{Response:}
%
Please note that there is already an overview of the LITS design in
Section 3.1.



\subsection*{2. Response to Review 4}

% --------
\qstart{R4W1,R4Revision1.} \emph{I know this is hard, but the
comparisons to other approaches isn't convincing. Wall clock
performance comparisons using different implementations in different
languages tuned for different hardware platforms/datasets only goes so
far.  Find a more convincing comparison metric and experiments, and do
the comparison.}
% --------

\answer{Response:}
%
We address the comment from the following angles:
%
\begin{list}{\labelitemi}{\setlength{\leftmargin}{5mm}\setlength{\itemindent}{-1mm}\setlength{\topsep}{0.5mm}\setlength{\itemsep}{0.5mm}\setlength{\parsep}{0.5mm}}

\item \emph{Same programming language}: All the compared solutions,
including the indexes that we obtained from github (i.e., ART, HOT,
SIndex, and LIPP), and the solutions that we implemented (i.e., RSS,
SLIPP, LITS), are written in C/C++.

\item \emph{Similar performance trend as reported in previous papers}:
Among the previous solutions, HOT has been shown to be the best
performing.  The HOT paper~\cite{HOT} shows that HOT has higher
throughput than ART.  The RSS paper~\cite{RSS} reports that HOT
achieves lower lookup times than both RSS and ART.  Our experiments
confirm previous results: HOT is the most competitive previous
solution.  The performance trend in our experiments is similar to
those reported in previous papers.

\item \emph{Representative data sets}:  We use 7 real-world and 4
synthetic string data sets in our experiments.  The 11 string data
sets cover a wide range of different distributions and
characteristics, as shown in Table~\ref{tab:datasets} and
Figure~\ref{fig:StringFeatures}.

\hspace{2mm} Moreover, HOT is the most competitive previous solution.
The HOT paper uses two string data sets, a url and an email data sets.
We also include a url data set and an email data set in our
experiments.

\hspace{2mm} Therefore, we believe that the data sets used in our
study are representative, and the performance difference due to tuning
for different data sets is low.

\item \emph{Three different hardware platforms}: We compare LITS, HOT,
and ART on three hardware platforms.  In addition to the default
machine with Intel Xeon Platinum 8380 CPUs, we also run experiments on
two different machines equipped with an Intel Core i7-4770 CPU and an
Intel Core i7-9700 CPU, respectively.  (Note that the HOT paper uses a
machine with an Intel i7-6700 CPU. We cannot find such a configuration
in our lab, but we try our best to obtain two machines with Intel i7
processors.)

\hspace{2mm} Due to space limitations, we add the new experimental
results in Appendix A.4 of the extended version of the
paper~\cite{litstr}.  Our results show that LITS achieves the best
performance for all the workloads across the three hardware platforms.

\item \emph{Tree height}: We report the index height as a metric that
is independent of the implementation languages and the hardware
platforms in (pp.10--11, Section~\ref{Re:R4O1}, paragraph on index
height).   Our results show that the height of LITS is significantly
smaller than HOT, ART, and SLIPP.  This partially explains the good
performance of LITS.

\end{list}


% --------
\qstart{R4W2.} \emph{What if the data distribution changes and the
table used for HPT doesn't work well anymore? How robust is it to
change?}
% --------

\answer{Response:}
%
In LITS, HPT is computed to approximate the conditional probabilities
$prob(c|{\mathcal{P}})$ for the string data set.  If the data
distribution changes, HPT may become less accurate, leading to
degraded index performance.  To handle data changes, LITS can sample
the index performance (e.g., for 1\% of the queries).  If it observes
that the index performance falls below a pre-defined water mark (e.g.,
50\% of the average performance after bulkloading), LITS can
judiciously retrain the HPT model and rebuild the entire index.  It
would be interesting future work to study how to lower or amortize the
rebuilding cost to reduce the impact on front-end index operations.
We add the description in (p.6, Section~\ref{R4W2}, paragraph on
dealing with data distribution changes).


\subsection*{3. Response to Review 5}

% --------
\qstart{R5W1,R5D10.} \emph{The major disadvantage of LIPP is that it
consumes much more memory space (i.e., space-inefficient) compared to
the other learned indexes. Since LITS is built based on LIPP, space
efficiency continues to be an outstanding weakness of the design (as
shown in Figure 10). However, there is no analysis regarding space
efficiency throughout the paper, and the discussion of the space
consumption results in the evaluation is undermined, providing no
insights. Please report the memory usage for the other learned
indexes.}
% --------

\answer{Response:}
%
First, we add Section~\ref{subsec:cost} in p.9 to analyze the time and
space costs of LITS.  The space cost of LITS excluding subtries is
$O(NlogN)$ for $N$ index entries.

Second, we modify (p.11, Section~\ref{Re:R5W1_R5D10}, paragraph on
space cost) and Figure~\ref{fig:BulkMem}.  We report space overhead of
all indexes except SLIPP, whose space cost exceeds 10GB in all four
datasets.

Finally, we describe the space consumption of SIndex, RSS, SLIPP, and
LITS in more details in Appendix A.6 of the extended version of the
paper~\cite{litstr}.


% --------
\qstart{R5W3.} \emph{Because LITS is built based on LIPP, a detailed
introduction to the LIPP structure should be included in Section 2 to
make the paper self-contained and to distinguish your contributions
from the ones in LIPP.}
% --------

\answer{Response:}
%
We modify (p.3, Section~\ref{Re:R5W3}, Paragraph on SLIPP) to describe
the main technique in LIPP.


% --------
\qstart{R5W4.} \emph{More theoretical analysis (e.g., a hash collision
analysis) is needed to understand the HPT's trade-offs between
accuracy and space.}

\answer{Response:}
%
In (p.6, Section~\ref{Re:R5W4}, Paragraph on analysis of HPT
accuracy), we analyze the accuracy of HPT in approximating conditional
probabilities.  Specifically, we describe the following theorem.  

\begin{customthm}{3.1}
%
If prefix ${\mathcal{P}}$ appears $n_{{\mathcal{P}}}$ times in the
string data set, and the HPT[$hash({\mathcal{P}})$] row sees $d$
occurrences of other prefixes, then 
%
\vspace{-1mm}
$$|HPT[hash({\mathcal{P}})][c].prob - prob(c|{\mathcal{P}})| \leq
\tfrac{1}{\tfrac{n_{{\mathcal{P}}}}{d}+1}.$$
%
\vspace{-3mm}
\end{customthm}

For a popular prefix ${\mathcal{P}}$, we expect $n_{{\mathcal{P}}} \gg
d$ with a reasonable sized HPT (e.g., 2MB).  In such cases, the
absolute error of the HPT approximation is small.  
%
Our experiments confirm this result.  For the string data sets in our
experiments, the average absolute error of the conditional probability
is 0.0006--0.006 for popular prefixes that appear at least 10,000
times.


% --------
\qstart{R5D1.} \emph{Section 3.1 lacks a discussion about how the data
structure handles a split of the compact leaf node.}

\answer{Response:}
%
The compact leaf node won't split in the sense of a B+-Tree node.
Instead, when an insert sees a full compact node (with 16 entries),
LITS performs the PMSS-based decision and replaces the compact node
with either a model-based node or a subtrie.  We have revised (p.5,
Section~\ref{Re:R5D1}, Paragraph 2).


% --------
\qstart{R5D2.} \emph{The key message in Section 3.2 is this: “the
existing linear models essentially assume that all prefixes appear
uniformly at random, and the distribution of the next character
following any given prefix is also uniform.” The math around this
statement is somewhat confusing.}

\answer{Response:}
%
In Equation~\ref{eqn:lm}, $\tfrac{s_{k+1}}{256}$ corresponds to
$\Sigma_{c=0}^{s_{k+1}-1}{prob(c|{\mathcal{P}}_{k})}$.
$\tfrac{s_{k+1}}{256}$ implies that any 8-bit character appears
uniformly at random.  Therefore, the existing linear models
essentially assume that the distribution of the next character
following any given prefix is uniform.  We have revised the
description in (p.5, Section~\ref{Re:R5D2}, Paragraph on problem of
existing linear models).


% --------
\qstart{R5D3.} \emph{Have you considered using a SIMD linear search
(instead of binary search) within a compact node? This may allow you
to have a larger compact node.}

\answer{Response:}
%
We implement a variant of LITS that exploits AVX512 to accelerate the
matching of hash codes in cnode.  However, our experiments show that
the improvement of search performance with SIMD is less than 1\%
across various data sets.  This is because cnode search is only a
small part of the overall search procedure.  LITS visits model-based
nodes from the root node to the parent of the cnode before reaching
the cnode.  After locating a matching hash code, LITS compares the
search key and the stored string key to verify the match.  Both the
tree traversal and the string key comparison are often more time
consuming than the search within the cnode.

We summarize the finding on SIMD acceleration for cnode search in
(p.12, Section~\ref{subsec:CNodePerf}, paragraph on variants of
compact node implementation).  Due to space limitations, we describe
the results in more detail in Appendix A.7 of the extended version of
the paper~\cite{litstr}.


% --------
\qstart{R5D4.} \emph{In Section 3.3, the authors claim that "In our
experiments, we find that the first method sees substantial space
waste for many string data sets because of the reserved empty slots.
Therefore, we choose the second method as the default design for the
compact node". This decision-making seems weird because the above
statement only covers half of the trade-offs. The other half is that
the second method could slow down insertions significantly. This is
neither evaluated nor discussed in the paper.}

\answer{Response:}
%
We report both the space cost and the insert throughput of the two
methods in the revision.  Our experimental results show that
preallocation incurs up to 93\% extra space overhead without
significant performance benefits.

We revise (p.7, Section~\ref{subsec:cnode}, paragraph on method to
support inserts) to describe both space and performance concerns.
Then, we summarize the experimental results on the space cost and
insert throughput in (p.12, Section~\ref{subsec:CNodePerf}, paragraph
on variants of compact node implementation).  Due to paper space
constraints, we describe the results in more detail in Appendix A.7 of
the extended version of the paper~\cite{litstr}.


% --------
\qstart{R5D5.} \emph{The numbers in Table 2 have no meanings. Are they
throughput numbers (Mops/s)?}
% --------

\answer{Response:}
%
Yes, the numbers in the table are throughput in Mops (i.e., million
operations per second).  We have added the metric, Mops, in the title
of Table~\ref{tab:LITPerf} in p.8.


% --------
\qstart{R5D6.} \emph{There is no evaluation/discussion regarding the
overhead of the GPKL computation.}
% --------

\answer{Response:}
%
We add (p.12, Section~\ref{Re:R5D6}, paragraph on GPKL computation
cost) to report the cost of GPKL computation.  Across all data sets,
a single invocation of the GPKL computation takes 0.8--1.7us.  The
total GPKL computation time contributes to 0.5\%--1.3\% of the total
insert time across all data sets.


% --------
\qstart{R5D7.} \emph{Why do you choose uniformly random instead of
Zipf in the YCSB evaluation? Do they have similar results?}
% --------

\answer{Response:}
%
In most experiments, we choose query keys uniformly at random because
the uniform distribution presents a more challenging scenario than the
zipf distribution for index operations.  Under the zipf distribution,
nodes that contain popular keys tend to stay in the CPU cache, leading
to higher index performance.

In the revision, we add a set of experiments for the zipf distribution
with zipf factor = 1.  First, we add the workload description in
(p.10, Section~\ref{subsec:setup}, paragraph 1).  Second, we report the
search performance in Figure~\ref{fig:DZ}, and the performance of more
YCSB workloads under the zipf distribution in Appendix A.5 in the
extended version of the paper~\cite{litstr}.  Third, we describe the
figure in (p.10, Section~\ref{subsec:perf}, paragraph 2--3). Finally,
we update the performance improvement numbers in
Section~\ref{subsec:perf} and in the abstract to include the zipf
experiments. 

Overall, the zipf results show similar trends as the results with the
uniform distribution.  LITS is the best performing index.


% --------
\qstart{R5D8.} \emph{LIPP is updatable. Why is SLIPP read-only in the
evaluation?}
% --------

\answer{Response:}
%
We implement the bulkload and the search operations for SLIPP.  Then,
we find that SLIPP has much worse search performance than HOT, ART,
and RSS.  Since SLIPP is clearly less competitive, we choose not to
implement the other operations for SLIPP to save development effort.
We omit SLIPP for the rest of the experiments.  We have revised (p.9,
Section~\ref{subsec:setup}, paragraph on SLIPP) to explain this point.


% --------
\qstart{R5D9.} \emph{According to Figure 9, the throughput numbers for
Workload F are higher than those for Workload A. This is a bit
suspicious because read-modify-write operations shouldn't be more
lightweight than reads/updates.}
% --------

\answer{Response:}
%
Thanks for pointing this out! We realize that our previous measurement
for the read-modify-write operations is erroneous.  A single
read-modify-write operation was mistakenly counted as two operations
(i.e. one read and one update), resulting in an inflated total query
count.  After correcting the problem, we rerun the tests for workload
F and update Figure~\ref{Re:R5D9} in p.10.


% --------
\qstart{R5D12.} \emph{There is a lot of repeated information in
Section 4.1 when introducing the baselines.}
% --------

\answer{Response:}
%
We have removed the redundant description of the baselines in Section~\ref{subsec:setup}.


% --------
\qstart{R5D13.} \emph{Typo: "We propose an optimized learn model" ->
"We propose an optimized learned model"}
% --------

\answer{Response:}
%
We have fixed the typo in (p.4, Section~\ref{Re:R5D13}, Paragraph on
optimized global HPT and local models).


